Graph Neural Network Flavor Tagger and measurement of $\mathrm{sin}2\beta$ at Belle II

We present GFlaT, a new algorithm that uses a graph-neural-network to determine the flavor of neutral B mesons produced in $\mathrm{\Upsilon(4S)}$ decays. We evaluate its performance using $B$ decays to flavor-specific hadronic final states reconstructed in a $362$ $\mathrm{fb}^{-1}$ sample of electron-positron collisions recorded at the $\mathrm{\Upsilon(4S)}$ resonance with the Belle II detector at the SuperKEKB collider. We achieve an effective tagging efficiency of $(37.40 \pm 0.43 \pm 0.36) \%$, where the first uncertainty is statistical and the second systematic, which is $18\%$ better than the previous Belle II algorithm. Demonstrating the algorithm, we use $B^0 \to J/\psi K_\mathrm{S}^0$ decays to measure the direct and mixing-induced CP violation parameters, $C = (-0.035 \pm 0.026 \pm 0.013)$ and $S = (0.724 \pm 0.035 \pm 0.014)$, from which we obtain $\beta = (23.2 \pm 1.5 \pm 0.6)^{\circ}$.

==> definitions.tex <==
% Packages
\usepackage{graphicx} % Include figure files
\usepackage{dcolumn} % Align table columns on decimal point
\usepackage{xcolor} % Color support
\usepackage{amsmath,amssymb} % Extended symbol collection
% \usepackage{hyperref} % Generate pdfs with hyperlinks
\usepackage[utf8]{inputenc} % Allow UTF8 characters
\usepackage[english]{babel} % All publications are in English
\usepackage[displaymath, mathlines]{lineno} % Line numbers for drafts
\usepackage{orcidlink} % for ORCIDs in author list
\usepackage[separate-uncertainty]{siunitx} % Handles units and unitful quantities
\usepackage{comment}

% Macros
\usepackage{belle2-particles}
\RequirePackage{relsize}

% useful commands for text sub- and superscripts
\newcommand{\Sub}[1]{\ensuremath{_{\text{#1}}}\xspace}
\newcommand{\Sup}[1]{\ensuremath{^{\text{#1}}}\xspace}

\def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\FourS {\Y4S}
\def\CP {\ensuremath{ C\!P}\xspace}

\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\def\B {\ensuremath{\PB}\xspace}

\usepackage{physics}

%%%%%%%%%%%%%%%%%%%%%%%%%
% set up ranges in siunitx
\renewcommand{\SIrange}[3]{\ensuremath{[\num{#1},\num{#2}]\,\si{#3}}\xspace}
\renewcommand{\numrange}[2]{\ensuremath{[\num{#1},\num{#2}]}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%% Commands specific to this analysis

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\belletwo{\mbox{Belle~II}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\lhcb {\mbox{LHCb}\xspace}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}

%% Software libraries
\newcommand{\softwarelibrary}[1]{\mbox{\textsc{#1}}\xspace}
\newcommand{\EvtGen}{\softwarelibrary{EvtGen}}
\newcommand{\Pythia}{\softwarelibrary{Pythia8}}
\newcommand{\KKMC}{\softwarelibrary{KKMC}}
\newcommand{\Geant}{\softwarelibrary{Geant4}}

% GFlaT
\newcommand{\gflat}{GFlaT\xspace}
\newcommand{\qrgflat}{\ensuremath{qr\Sub{\!\gflat}}\xspace}

% tag and sig
\newcommand{\sigsub}{\text{sig}}
\newcommand{\tagsub}{\text{tag}}

% Bsig and Btag (without charges)
\defParticleAndAntiparticle{Bsig}{B}{\sigsub}{}
\defParticleAndAntiparticle{Btag}{B}{\tagsub}{}
% with explicit charges
\defParticleAndAntiparticle{Bzerosig}{B}{\sigsub}{\Pnumeral{0}}
\defParticleAndAntiparticle{Bzerotag}{B}{\tagsub}{\Pnumeral{0}}

\defParticleAndAntiparticle{Bzerox}{B}{x}{\Pnumeral{0}}


% flavor tags
\newcommand{\qsig}{\ensuremath{q_{\sigsub}}\xspace}
\newcommand{\qtag}{\ensuremath{q_{\tagsub}}\xspace}

% efficiency asymmetries
\newcommand{\asig}{\ensuremath{a_{\sigsub}}\xspace}
\newcommand{\atag}{\ensuremath{a_{\tagsub}}\xspace}

% effective tagging efficiency
\newcommand{\efftag}{\ensuremath{\varepsilon_{\tagsub}}\xspace}

% efficiency
\newcommand{\effi}{\ensuremath{\varepsilon_i}\xspace}

% average wrong-tag rate
\newcommand{\wavg}{\ensuremath{\bar{w}}\xspace}

% S and C (CP)
\newcommand{\SCP}{\ensuremath{S}\xspace} 
\newcommand{\CCP}{\ensuremath{C}\xspace} 

% DGCNNs
\newcommand{\EdgeConv}{\textsc{EdgeConv}\xspace}

% sign function
\DeclareMathOperator{\sign}{sign}

\def\sWeight{\mbox{\em sWeight}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%

